Revisiting Event Horizon Finders

Event horizons are the defining physical features of black hole spacetimes, and are of considerable interest in studying black hole dynamics. Here, we reconsider three techniques to localise event horizons in numerical spacetimes: integrating geodesics, integrating a surface, and integrating a level-set of surfaces over a volume. We implement the first two techniques and find that straightforward integration of geodesics backward in time to be most robust. We find that the exponential rate of approach of a null surface towards the event horizon of a spinning black hole equals the surface gravity of the black hole. In head-on mergers we are able to track quasi-normal ringing of the merged black hole through seven oscillations, covering a dynamic range of about 10^5. Both at late times (when the final black hole has settled down) and at early times (before the merger), the apparent horizon is found to be an excellent approximation of the event horizon. In the head-on binary black hole merger, only {\em some} of the future null generators of the horizon are found to start from past null infinity; the others approach the event horizons of the individual black holes at times far before merger.

==> Makefile <==
#-----------------------------------------------------------------------
# $Id:$
#-----------------------------------------------------------------------
FIGURES=figure10.eps figure11.eps figure12.eps figure13.eps figure14.eps\
	figure15.eps figure1.eps figure2.eps figure3.eps figure4.eps\
	figure5a.eps figure5b.eps figure6.eps figure7a.eps figure7b.eps\
	figure8a.eps figure8b.eps figure9a.eps figure9b.eps figure9c.eps \
	figure9d.eps

all: paper.dvi

balooney:
	latex paper.tex

paper.dvi: paper.tex $(FIGURES) balooney
	latex paper
	latex paper

paper.ps: paper.dvi
	dvips -N0 -P pdf -t letter -o paper.ps paper.dvi

paper.pdf: paper.ps 
	ps2pdf paper.ps

# Automatically make postscript .eps files from .agr files
# The 'epsfig.eps' and the includefonts.tex stuff are there
#  to include the correct fonts in the eps files.
# If your agr files use no special fonts, only the first line is necessary.
%.eps:%.agr
	xmgrace -hardcopy -hdevice EPS -printfile epsfig.eps $<
	latex includefonts.tex
	dvips -E includefonts.dvi -o $@
	rm epsfig.eps

%.eps:%.png
	convert $< eps3:$@

# Automatically make postscript .eps files from .fig files
%.eps:%.fig
	fig2dev -L eps $< $@

# The || : is there to make sure that subsequent lines get executed even if
# some of the removes fail because the files to be removed do not exist.
clean:
	rm *.aux || :
	rm *.dvi || :
	rm *.log || :
	rm *.bbl || :
	rm *.blg || :
	rm $(FIGURES) || :

